Fast Conical Hull Algorithms for Near-separable Non-negative Matrix Factorization

The separability assumption (Donoho & Stodden, 2003; Arora et al., 2012) turns non-negative matrix factorization (NMF) into a tractable problem. Recently, a new class of provably-correct NMF algorithms have emerged under this assumption. In this paper, we reformulate the separable NMF problem as that of finding the extreme rays of the conical hull of a finite set of vectors. From this geometric perspective, we derive new separable NMF algorithms that are highly scalable and empirically noise robust, and have several other favorable properties in relation to existing methods. A parallel implementation of our algorithm demonstrates high scalability on shared- and distributed-memory machines.

==> parallel.tex <==
The computation of the NMF of $\vX{}$ can be decomposed into three phases:
initialization, topic selection, and refitting.
%
In this section, we briefly describe our approach to parallelizing these three
phases.
%
In particular, we discuss two approaches --- sparse and dense --- to computing
$\vQ$, which takes up the majority of the compute time.
%
For brevity, we refer to our algorithm as \texttt{Conic}.

\subsubsection{Initialization}
%
Throughout \texttt{Conic}, $\vX^T\vX$ and three norms ($\|\vX\|^2_{fro}$,
$\|\vx_i\|_{2}$, and $\|\vx_i\|_{1}$, where $\vx_i\in{}\vX$) are repeatedly
used.
%
Typically, $\vX$ is sparse and therefore, efficient parallelization of 
$\vX^T\vX$ is non-trivial; in fact, parallel sparse matrix-matrix computation
is the subject of many ongoing research studies~\cite{Buluc:2011}.
%
In our implementation, we compute $\vX^T\vX$ as a series of parallel
\emph{rank-1} updates of the $C^n_2$ combinations of the columns of $\vX$.
%
Computation of the three norms requires a single pass over $\vX$; therefore, it
requires accessing $nnz(\vX)$ elements and $O(nnz(\vX)$ operations.
% 
Parallelizing the computation of these quantities is achieved by splitting the
computation by columns of $\vX$.
%
As $n\ggg{}P$, where $n$ is the number of columns in $\vX$ and where $P$ is the
total number of cores, splitting along the colummns of $\vX$ ensures each cores
gets sufficient work.
%
In typical applications, $m$ grows much faster than $n$; this allows us to
compute $\vX^T\vX$ just once and perform a \emph{rank-1} update of $\vX^T\vX$
when $m$ changes.

\subsubsection{Topic Selection}
\label{subsec:compute_Q}
In \texttt{Conic}, topic selection is carried out by first computing 
$\vQ_{n,n}$, an intermediate matrix, which is computed for each of the $r$
topics; to recap, $\vQ = max(\vX^T\vX-\vH^T(\vX^T\vX)_A, 0)$.
%
Once $\vQ$ is computed, various selection strategies can be applied to pick the
next topic; for example, picking $max(\|\vq_i\|_2^2/\|x_i\|_2^2)$, where
$\vq_i$ and $\vx_i$ represent the columns of $\vQ$ and $\vX$ respectively, is
one such approach.
%
The number of positions of $\vQ$ that need to be computed is exactly
$nnz(\vX^T\vX)$, where each update takes $O(r)$ operations.
%
Efficient computation of $\vQ$ depends on the structure of $\vX^T\vX$.
%
When $\vX^T\vX$ is sparse, then $\vQ$ can be computed as a series of
$nnz(\vX^T\vX)$ updates, where each update to is an inner-product of row
$\vH^T_{i,:}$ with column $(\vX^T\vX_A)_{:,j}$.
%
This computation can be parallelized over the $n$ columns of $\vQ$.
%
However, as the non-zero entries of $\vX^T\vX$ are not distributed evenly
across all columns, a naive division of parallel work will lead to load
imbalance.
%
Therefore, we use a dynamic task scheduling algorithm, in which we recursively
divide the space of $n$ columns with a base case of $k$, where $k\lll{}p$.
%
Each core repeatedly computes $k$ contiguos columns of $\vQ$ at a time before
retrieving the next set of $k$ columns to update.
%
This sparse approach to computing $\vQ$ is also space efficient as $\vQ$ is 
never explicitly materialized.
%
When, $\vX^T\vX$ is relatively dense, then $\vQ$ can be computed as a
\emph{rank-k} update to the $\vQ$, where the update is of the form $\vQ = \vQ -
\vH^T(\vX^T\vX)_A$ --- this can be computed efficiently using the 
BLAS-3~\cite{Dongarra:1990:BLAS3} operation \func{dgemm}.
%
Although dense updates result in wasted operations corresponding to 
zero-entries of $\vX^T\vX$, updating $\vQ$ in this manner is sometimes more
efficient because \func{dgemm} has good memory to computation ratio ($O(n^3)$
computations with $O(n^2)$ memory accesses).
%
Parallelization of the dense updates can be done by 
splitting up the columns of $n$ into $k$ nearly even chunks. 
%
Each chunk of $k$ columns is updated by a \emph{rank-k} update with the
corresponding $k$ rows of $\vH^T$ and $k$ columns of $(\vX^T\vX)_A$.
%
Unlike the sparse updates, we can schedule the cores statically as the load is
balanced across as the chunks.
%
However, computing $\vQ$ using \func{dgemm} requires explicit materialization 
of $\vQ$, which requires $O(n^2)$ extra space.

\subsubsection{Refitting}
\label{subsec:refit}
%
At each iteration, after a topic is picked, the entire matrix $\vH$ is refitted
iteratively using a coordinate descent-like method.
%
This refitting step itself goes through multiple inner iterations where each 
inner iteration consists of looping over the $r$ selected topics and performing
vector updates to the rows of $\vH$.
%
Although this operation has a sequential dependency from one inner iteration to
the next, each inner iteration is parallelized over the space of the $n$
columns of $\vH$ that need to be updated.
%
Currently, we always refit $\vH$ using dense operations as all the matrices
($\vH, (\vX^T\vX)_A, \vU$) are $(n,r)$ and can be easily held in memory without
loss of performance.
%
In fact, we maintain $\vH$ and $(\vX^T\vX)_A$ in both row-major and
column-major format because computing $\vQ$ benefits from row-major
representation and the refitting phase benefits from column-major
representation.
%
\paragraph{Caveat}
%
The refitting step largely consists of a few element-wise operations on the
columns of $\vH$, an inner-product between $(\vX^T\vX)_{A_i}$ and $\vH_i$,
and finally, a \emph{rank-1} update of $\vU$ to reflect changes in the columns
of $\vH$.
%
All these operations have poor computation to memory ratio; therefore, the 
refitting step is largely memory-bandwidth bound.
%
This is especially true of the \emph{rank-1} update, which grows increasingly
compute intensive with the addition of new topics.
%
To wit, when there are $r$ topics, there are $r$ coordinates to iterate over 
in the inner loop; each iteration results in a \emph{rank-1} update to $\vU$,
which is a $\R^{nxr}$ matrix.
%
In our implementation, we use dense matrix operations during the refitting 
step.
%
While this is acceptable for most matrices, for matrices that are extremely
sparse, it is beneficial to refit $\vH$ in a sparse manner.
%
Consider the matrices that are involved in the refitting step.
%
$\vH$ is initialized to $\emptyset{}$ and with the addition of each new topic,
a new column is added to $\vH$. 
%
The sparsity structure of this new column, say $i$, is exactly the same 
as the sparsity structure of $(\vX^T\vX)_{A_i}$.
%
Furthermore, $\vU$ is a linear combination of the columns of $\vH$ scaled by
the columns of $\vS$.
%
Consequently, for each non-zero entry in $\vH$, there is a corresponding
non-zero entry in \emph{each} column of $\vU$; in fact, each column of $\vU$
has identical sparsity structure.
%
Therefore, refitting using a sparse representation does not require any changes
to the sparsity structure of either $\vH$ or $\vU$.
%

\subsubsection{Experiments}
\label{subsec:implementation}
%
We implemented a shared- and distributed-memory parallel version of
\texttt{Conic} in \Cpp{}.
%
That is, our implementation can exploit parallelism when running on multi-core
machines, or on clusters of multi-core machines.
%
For shared-memory parallelism, we use PFunc~\cite{kambadur09:pfunc}, a
lightweight and portable library that provides C and \Cpp{} APIs to express
task parallelism.
%
For distributed-memory parallelism, we use MPI~\cite{MPI-1,MPI-2}, a popular
library specification for message-passing that is used extensively in
high-performance computing.
%
Our implementation handles both the sparse and dense versions of the updates
to $\vQ$ as described in Section~\ref{subsec:compute_Q} --- the choice of the
version can be made depending on the sparsity of $\vX^T\vX$.
%

\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|} 
\hline
Name & D & W & nnz($\vX$) & nnz($\vX^T\vX$) & Sparsity & Time(R=100) & Memory \\
\hline
RCV1 & 781265 & 43001 & 59.16e06 & 172.3e06  & 5\% & 409 secs & 3.6 GB\\
\hline
PPL2 & 351849 & 44739 & 19.43e06 & 1.99e09 & 99.8\% & 1147 secs & 30.2 GB\\
\hline
IBMT & 124708 & 25998 & 1.03e06 & 1.77e06 & 0.2\% & 9.8 secs & 1 GB\\
\hline
\end{tabular}
\caption{Statistics of the datasets that were used in our experiments.  $\vX$
refers to the word-document matrix and $\vX^T\vX$ refers to the word-covariance
matrix. RCV1 and IBMT are factorized using sparse matrix operations, whereas
PPL2 is factorized using dense matrix operations. The times reported are for
R=100 on eight cores on \texttt{daniel}.} 
\label{tbl:datasets}
\end{table*}
%
%
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth,height=0.7\linewidth]
{figures/scalability/daniel.eps}
\caption{Multi-core speedup of RCV1, IBMT, and PPL2 datasets when running on
\texttt{daniel}. All times are for R=100.}
\label{fig:pfunc}
\end{figure}
%
%
To test the multi-core performance and scalability of \texttt{Conic}, we ran
experiments on \texttt{daniel}, a dual-socket, quad-core Intel\textregistered{}
Xeon\texttrademark{} X5570 machine with 64GB of RAM running Linux Kernel
2.6.35-24 (total 8 cores).
%
For compilation, we used GCC v4.4.5 with: ``\texttt{-O3 -fomit-frame-pointer
-funroll-loops}'' in addition to PFunc 1.02, OpenMPI 1.4.5 and untuned ATLAS
BLAS.
%
We ran large-scale experiments on three datasets: RCV1~\cite{RCV1},
co-occurence matrix of people and places from ClueWeb09 (PPL2)
Dataset~\cite{PPL2}, and IBM Twitter (IBMT) dataset. 
%
The statistics relating to these three large datasets are presented in 
Table~\ref{tbl:datasets}.
%
Datasets RCV1 and IBMT were run with the sparse version, whereas PPL2 was 
run with the dense version.
 
%
Figure~\ref{fig:pfunc} depicts the multi-threaded performance of our
implementation on \texttt{daniel} while detecting 100 topics.
%
Our implementation is able to factorize RCV1 in 409 seconds on 8 cores and
achieve $4.2x$ speedup over 8 threads when compared to the sequential
implementation.
%
Similarly, for IBMT we achieve $4.5x$ speedup, while completing the
factorization in $9.8$ seconds on 8 cores.
%
The reason for the sub-linear speedup is two-fold.
%
First, as we compute $\vQ$ using sparse matrix operations and we do not tune
the layout of data, we are limited by the memory bandwidth.
%
Second, in the sparse version, we currently refit $\vH$ using dense vector and
matrix operations, which is sub-optimal as it encumbers wasted computations and
memory operations.
%
This is especially true of hyper-sparse datasets such as IBMT, which has only
$0.2\%$ non-zeros in $\vX^T\vX$.
%
We believe that we can improve scalability by switching to a sparse version for
refitting and by careful alignment of data so as to increase memory bandwidth.
%
For the dense case, we are able to factorize PPL2 in 1147 seconds with just 8
cores.
%
Although PPL2 shows good scalability ($5x$ over eight cores), we believe that
we can further improve both the scalability and the raw performance by
switching to a version of BLAS tuned to our systems and by replacing some of
the level-1 and level-2 BLAS operations, which have poor memory-to-compute
ratio, with level-3 BLAS operations, which have a better memory to compute
ratio.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% UNCOMMENT HERE FOR RESULTS ON OXYGEN
%\begin{figure}
%\centering
%\includegraphics[width=0.8\linewidth,height=0.7\linewidth]
%{figures/scalability/oxygen.eps}  
%\caption{Multi-node speedup of RCV1 and PPL2 datasets when running on
%\texttt{oxygen} cluster. IBMT was not run as it was too small to run on
%\texttt{oxygen}. All times are for R=50.}
%\label{fig:mpi}
%\end{figure}
%
%
%To test the multi-core performance and scalability of \texttt{Conic}, we ran
%experiments on \texttt{oxygen}, a six-node cluster of dual-socket, quad-core
%Intel\textregistered{} Xeon\texttrademark{} E5410 machine with 32GB of RAM
%per-node running Linux Kernel 2.6.31-23 (total 48 cores).
%
%For compilation, we used GCC 4.4.1 with: ``\texttt{-O3 -fomit-frame-pointer
%-funroll-loops}'' in addition to PFunc 1.02, OpenMPI 1.4.5 and untuned ATLAS
%BLAS.
%
%Figure~\ref{fig:mpi} depicts the multi-node (cluster) performance of our
%implementation on \texttt{oxygen}; the number of threads per process was set to
%8 and the number of topics was 50.
%
%We did not include IBMT in these experiments as it is too small a dataset to
%run on a cluster.
%
%We see that the scaling for RCV1 and PPL2 is similar to that of multi-core
%machines (Figure~\ref{fig:pfunc}).
%%
%The reason for sub-linear scalability in a cluster setting is also two-fold.
%
%When running on a cluster, we partition and store only a subset of the dataset
%and matrices on each process.
%
%While this is necessary to maintain a flat memory-profile as we increase the
%number of processes,  it introduces additional global communication and
%synchronization operations at the end of each iteration.
%
%Another contributing factor to the scalability in a cluster is load balancing.
%
%While we dynamically load balance computations amongst threads within a single
%node, such a scheduling scheme is impractical to pursue in distributed-memory
%machines.
%
%Instead, work is partitioned \textit{apriori} based on data ownership, which
%introduces load imbalance.
%
%For example, in the sparse version, each processor can have a might have a
%different number of non-zeros (computations).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\Anju{I think we should at least mention a sentence or two on the performance 
of \texttt{Conic} on distributed-memory machines.}

%
%
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}  \hline

\multirow{2}{*}{Dataset} & 
\multicolumn{4}{|c|}{Conic (secs)} &
\multicolumn{3}{|c|}{BRRT (secs)} \\ \cline{2-8}
 & R=10 & R=25 & R=50 & R=100 & E=3 & E=5 & E=10 \\
\hline
IBMT & 0.08 & 0.38 & 1.78 & 9.8 & 190.8 & 348.4 & 636.9 \\ \hline
RCV1 & 4.2 & 15.4 & 67.2 & 409 & 1183.7 & 1883.6 & 3749.5 \\ \hline
PPL2 & 67.2 & 196 & 443.8 & 1147 & 1135.2 & 1892.7 & 3913.7 \\ \hline
\end{tabular}
\caption{Running times of \texttt{Conic} versus BRRT. All experiments were run
on \texttt{daniel} with 8 threads. R and E represent the number of topics and
epochs, respectively. \textcolor{red}{BRRT is invariant in R, but its accuracy
is dependent on E.} Timing results for BRRT were obtained with R=10.
\texttt{Conic} discovers one topic per-iteration; hence, its running time is
dependent on R.}
\label{tbl:comp}
\end{table*}
%
%
To compare our performance against the state-of-the-art BBRT algorithm, we ran
their algorithm on \texttt{daniel} with the options ``\texttt{--dual 0.01
--epochs 10 --splits 8 --hott <R> --normse 1 --primal 0.0000001}''; the source
code and the parameters were graciously provided by the authors.
%
A detailed comparison of the results obtained is shown in Table~\ref{tbl:comp}.
%
A head-to-head comparison is difficult because of the different characteristics
of BRRT and \texttt{Conic}.
%
\textcolor{red}{For example, BRRT's runtime is not dependent on R, the number
of topics, but it's accuracy is dependent on E, the number of epochs --- the
numbers listed in Table~\ref{tbl:comp} for BRRT are for R=10.}
%
\texttt{Conic} finds one topic per iteration, and therefore, its running time
is dependent on the R.
%
For IBMT and RCV1, which are sparse datasets, we see that \texttt{Conic}
performs quite well when compared to BRRT, especially for small values of R.
%
The performances for PPL2 are comparable when R=100 and E=3; we attribute this
to the fact that \texttt{Conic} uses both untuned BLAS and it's performance
could be improved further as mentioned before.
%
\Anju{It would be fair to say that there is a cross-over point (at least for 
dense datasets) where BRRT would start performing better than \texttt{Conic}.
However, this crossover point would be dependent on the dataset. We should do
a thorough complexity analysis of our algorithm somewhere.}
%
\Anju{It is not quite true that BRRT's running time is invariant in R --- I
have a hunch that its convergence does depend on R even though its per-epoch
time does not depend on R. I don't know BRRT well enough --- any comments?
If you agree, we need to change the text in \textcolor{red}{red}.}

